Storage Sizing and Placement through Operational and Uncertainty-Aware Simulations

As the penetration level of transmission-scale time-intermittent renewable generation resources increases, control of flexible resources will become important to mitigating the fluctuations due to these new renewable resources. Flexible resources may include new or existing synchronous generators as well as new energy storage devices. Optimal placement and sizing of energy storage to minimize costs of integrating renewable resources is a difficult optimization problem. Further,optimal planning procedures typically do not consider the effect of the time dependence of operations and may lead to unsatisfactory results. Here, we use an optimal energy storage control algorithm to develop a heuristic procedure for energy storage placement and sizing. We perform operational simulation under various time profiles of intermittent generation, loads and interchanges (artificially generated or from historical data) and accumulate statistics of the usage of storage at each node under the optimal dispatch. We develop a greedy heuristic based on the accumulated statistics to obtain a minimal set of nodes for storage placement. The quality of the heuristic is explored by comparing our results to the obvious heuristic of placing storage at the renewables for IEEE benchmarks and real-world network topologies.

==> Inter.tex <==
First, we note that Fig.~\ref{fig:ErrorP} demonstrates the effectiveness of node-specific control for mitigating the impact of renewable generation fluctuations on the network.  The upper curve in the inset in Fig.\ref{fig:ErrorP} shows the level of constraint violations for a system that maintains generation-load balance purely via proportional control, i.e. only the controlled generators responding to a generation-load imbalance in proportion to their capacity.  Without the node-specific control in our model of energy storage, the response of the generators is inflexible, and system begins to experience constraint violations for small values of renewable penetration.  With the node-specific control allowed by our storage model, Figure~\ref{fig:ErrorP} shows that the control can eliminate all constraint violations up to about 30\% renewable penetration for all the node configurations we explored.  We do not attribute this behavior to the storage itself, rather, this appears to be a property of the flexibility of node-specific control.  Although we did not explore this possibility, we believe that if we would have incorporated the controlled generators $\G$ into our control algorithm, we would have seen similar performance up to a renewable penetration of 30\% for a system without any storage.  It is interesting to note that more detailed studies have found similar thresholds for renewable penetration\cite{Meibom2010}.  

Figure~\ref{fig:Cuts} shows the location of the nodes with storage in the reduced-node sets identified by our heuristic in algorithm~\ref{alg:OptPlace}.  The two-node set is perhaps the most illustrative of how optimal placement and sizing of storage in a network does yield itself to simple rules of thumb or intuition.  Intuition may have led to the conclusion that storage should be placed at the site of the fluctuating renewables because it can effectively mitigate the fluctuating power flows without these flows ever being injected into the network.  It seems plausible that this should lead to a minimal amount of storage and quality control, however, the results in Fig.~\ref{fig:Cuts} and \ref{fig:ErrorP} show otherwise.  The nodes in the two-node set do not include either of renewable generation sites.  In fact, even when expanded to the ten-node set, only one of the three renewable sites is included.  These results demonstrate that the nodes that have a high degree of control over congestion caused by renewable fluctuations are not necessarily the renewable nodes themselves.

To further demonstrate this point, we performed an additional simulation where the reduced-note set included just the three renewable sites. Figure~\ref{fig:ErrorP} shows that the quality of control over the constraint violations is the same for this handpicked case as in the two-, ten-, and unrestricted-node sets.  Figures~\ref{fig:EnergyCapP} and \ref{fig:PowerCapP} help to distinguish between these node sets.  For renewable penetrations below about 30\%, the network total power capacity and energy capacity of the storage is nearly the same for each case.  Beyond 30\% where we begin to see a few constraint violations in Fig.~\ref{fig:ErrorP}, the two-node set shows significantly lower total network power and energy capacity compared to the ten or unrestricted-node cases.  The handpicked case is comparable to the ten-node case.  A lower network total capacity implies that the nodes identified in the two-node case have the highest degree of controllability over the network congestion caused by the fluctuating renewables.

A possible reason for the two-node set showing better controllability is evident from Fig.~\ref{fig:Cuts}.  These two nodes sit at the end or the middle of crucial transmission lines that link two major regions in RTS-96.  In reference to Fig.~\ref{fig:Cuts}, we name these regions ``upper'' and ``lower''.  We conjecture that by controlling the power injections at these nodes, our control scheme can effectively control to which region the renewable generation is directed.  Therefore, our control can direct the renewable fluctuations to the region that, at that point in time, has the greatest ability to assist in mitigation.  In addition to simply absorbing the fluctuations locally, the storage may be used to redirect the renewable fluctuations throughout the network to leverage other resources to assist in the control.
